In-context Pretraining: Language Modeling Beyond Document Boundaries

Large language models (LMs) are currently trained to predict tokens given document prefixes, enabling them to directly perform long-form generation and prompting-style tasks which can be reduced to document completion. Existing pretraining pipelines train LMs by concatenating random sets of short documents to create input contexts but the prior documents provide no signal for predicting the next document. We instead present In-Context Pretraining, a new approach where language models are pretrained on a sequence of related documents, thereby explicitly encouraging them to read and reason across document boundaries. We can do In-Context Pretraining by simply changing the document ordering so that each context contains related documents, and directly applying existing pretraining pipelines. However, this document sorting problem is challenging. There are billions of documents and we would like the sort to maximize contextual similarity for every document without repeating any data. To do this, we introduce approximate algorithms for finding related documents with efficient nearest neighbor search and constructing coherent input contexts with a graph traversal algorithm. Our experiments show In-Context Pretraining offers a simple and scalable approach to significantly enhance LMs'performance: we see notable improvements in tasks that require more complex contextual reasoning, including in-context learning (+8%), reading comprehension (+15%), faithfulness to previous contexts (+16%), long-context reasoning (+5%), and retrieval augmentation (+9%).

==> algorithm/alg1.tex <==



% \begin{algorithm}
% \caption{Path Cover Algorithm }
% \label{alg1}
% \hspace*{\algorithmicindent} \textbf{Input}: Document graph $\mathcal{G} =(\mathcal{D}, \mathcal{L})$, $N(d_i)$ returns a list of nearest neighbor documents for $d_i$\\
% \hspace*{\algorithmicindent} \textbf{Output}: List of paths $P$=$\{p\}$ covering the graph
% \begin{algorithmic}[1]
%   % \STATE $P \gets$ list()
%   % \STATE $d_i \gets$ None
%   \WHILE{$|\mathcal{D}| > 0$}
%     \STATE $d_i \gets $ \texttt{Min\_Degree} ($\mathcal{D}$)
%     \COMMENT{Choose a minimum degree unvisited document}
%     \STATE $p \gets [d_i]$
%         \COMMENT{initialize a new path $p$ starting from $d_i$}
%      \WHILE[Continue if there exists a neighbor $d_j$ hasn't been visited] {$\exists d_j \in N(d_i)$ in $\mathcal{D}$ }
%         \STATE $d_i \gets d_j$ 
%         \STATE $p.append(d_i)$ 
%                 \COMMENT{Add the document to the current path $p$}
%         % \COMMENT{Add the document to the current path $p$}
%         \STATE $\mathcal{D}.remove(d_i)$ 
%      \ENDWHILE
%     \STATE $P.append(p)$ \COMMENT{Add $p$ to list of paths}
%   \ENDWHILE
%   \RETURN{$P$}
% \end{algorithmic}
% \end{algorithm}

  \begin{wrapfigure}{b}{0.48\textwidth}
    \begin{minipage}{0.48\textwidth}
    \begin{algorithm}[H]
\caption{Minimum Path Cover Algorithm}
\label{alg1}
% \hspace*{\algorithmicindent} 
\textbf{Input}: Document graph $\mathcal{G} =(\mathcal{D}, \mathcal{L})$ \\
\hspace*{2\algorithmicindent}  $N(d_i)$ returns nearest neighbors for $d_i$ \\
\hspace*{2\algorithmicindent}  $\texttt{min\_deg}(\mathcal{D})$ returns a min-degree doc \\
% \hspace*{\algorithmicindent} 
\textbf{Output}: Path cover $P$
\begin{algorithmic}[1]
\small
 \STATE $P \gets \phi$ 
  \WHILE{$|\mathcal{D}| > 0$}
    \STATE $d_i \gets \texttt{min\_deg}(\mathcal{D})$  
    % \footnotesize\ttfamily\textcolor{blue}{\# Return a min-degree unvisited doc}
    \STATE $p \gets [d_i]$  \COMMENT{Initialize path $p$ from $d_i$}
    \WHILE{$\exists d_j \in N(d_i)$ in $\mathcal{D}$ }
        \STATE $d_i \gets d_j$
        \STATE $p.append(d_i)$
        \STATE $\mathcal{D}.remove(d_i)$
     \ENDWHILE
    \STATE $P.append(p)$
  \ENDWHILE
  % \RETURN{List of paths $P=\{p\}$ covering the graph}
  \RETURN{$P$}
\end{algorithmic}
\end{algorithm}
    \end{minipage}
  \end{wrapfigure}


==> section/intro.tex <==
\section{Introduction}
% Large language models (LMs)~\citep{openai2023gpt4, touvron2023llama} have demonstrated impressive capabilities in performing downstream tasks via prompting: LMs generate text completions based on task-specific details formatted as input contexts. These contexts can encompass various information, including task instructions, in-context learning examples, and documents. The ability of LMs in interpreting these contexts is crucial for diverse applications, ranging from instruction-following~\citep{ouyang2022training} and conversational interfaces to reading comprehension~\citep{zhang2020machine}, in-context learning~\citep{NEURIPS2020_1457c0d6}, and the integration of external knowledge from search engines and datbases~\citep{shi2023replug}. Despite their potential, recent studies highlight that LMs can sometimes struggle to understanding context. This limitation leads to several challenges such as failure to follow instructions~\citep{mckenzie2023inverse, Efrat2020TheTT}, difficulties in reasoning over documents~\citep{liu2023lost, shi2023large}, and instability in in-context learning performance~\citep{zhao2021calibrate}. 
% \weijia{start with the problem of contexts: LMs learn to predict tokens given the , allowing them to have the cool ....}
Large language models (LMs) learn to generate text completions based on input contexts such as task instructions, examples, and chat histories, allowing them to excel in diverse applications including instruction-following~\citep{ouyang2022training}, conversational interfaces, reading comprehension~\citep{zhang2020machine}, and in-context learning~\citep{NEURIPS2020_1457c0d6}.
Despite their success, recent studies highlight that LMs sometimes struggle to understand the context.
This limitation poses several challenges such as failure to follow instructions~\citep{mckenzie2023inverse, Efrat2020TheTT, memotrap}, difficulties in reasoning over documents~\citep{liu2023lost, shi2023large}, and instability in in-context learning performance~\citep{zhao2021calibrate}. 
We hypothesize that the LMs' insufficient understanding of contexts can be attributed in part to the current pretraining approach~\citep{openai2023gpt4, touvron2023llama} which only considers text from a single document and thus provides limited contexts for the model to learn from. 
In this work, we present \model, a new pretraining method that places semantically relevant documents in a coherent input context during pretraining, thereby exposing language models to longer contexts and providing pretraining signals beyond document boundaries.

Several studies have shown the benefit of pretrain language models on a small-scale related document
As shown in Figure \ref{fig:intro}, when predicting the following tokens for the phrase "\textcolor{brilliantrose}{\textit{For 2022, FIFA set the prize money at \$42m,}}" LMs could reference prior documents stating "\textcolor{brilliantrose}{\textit{World Cup never awarded more than \$10M before 2022}}" and learn to infer that "\textcolor{brilliantrose}{\textit{the highest so far}}". As \model only changes document ordering during pretraining, it can be easily integrated into existing pretraining pipelines for large-scale LMs. \weijia{give more details here}

\weijia{2. challenges. 3. methods .. 4. related works}
Constructing such coherent input contexts introduces two challenges: (1) comparing pairwise document similarity in the pretraining corpus, especially web-scale corpus that contain millions of documents, is intractable. (2) It is crucial to ensure that every document from the corpus is included at its original frequency during pretraining, thereby maintaining its original pretraining data distribution. To handle this computation on a web-scale pretraining corpus, we employ a retriever model paired with an efficient search index, allowing us to pair each document with its nearest neighbor documents even in billion-scale corpus. We then formulate the second challenge as a document graph traversal problem for which we develop an effective algorithm that ensures that each document is included in the pretraining batches in its original frequency.


To evaluate the effectiveness of \model, we pretrained language models from 0.3 to 7 billion parameters
% Each model has an 8192-token length context window and is pretrained 
on 300 billion tokens from the Commoncrawl dataset~\citep{wenzek2020ccnet}. Across all model scales, the \model LMs 
(\modelname)
% \textbf{I}n-context \textbf{P}retrained \textbf{L}anguage \textbf{M}odels (\modelname) 
demonstrate strong language modeling and downstream tasks performance, significantly outperforming the LMs pretrained using the standard approach 
on the same corpus. 
We observe various benefits brought by \model:
(1) \textbf{better in-context learning} with an average increase of 8\% across 8 datasets; (2) \textbf{improved reading comprehension}, with an average of 14.9\% improvement on 8 reading comprehension tasks;  (3) \textbf{more faithful} to prior contexts (+15.9\%);  (4) \textbf{better long context reasoning},  showing a 4.9\% boost.; and (5) \textbf{better retrieval augmentation}, leading to 9.3\% gains when 
augmenting them with external knowledge such as documents retrieved from Wikipedia. 
Our results demonstrate that \model, by simply altering order of the pretraining documents, offers a scalable and simple approach to significantly enhance LMs' capabilities of understanding and reasoning over contexts.

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{fig/intro.png}
    \caption{\textbf{Overview of \model}. Different from the \textit{standard} pretraining strategy that place randomly shuffled documents in the input context, \model places related documents in the same contexts, making models learn to reason across prior documents. For example, when predicting the following tokens for the phrase "\textcolor{brilliantrose}{\textit{For 2022, FIFA set the prize money at \$42m,}}" LMs could reference prior documents stating "\textcolor{brilliantrose}{\textit{World Cup never awarded more than \$10M before 2022}}" and learn to infer that "\textcolor{brilliantrose}{\textit{the highest so far}}". 
    \weijia{get rid of quesiton mark: in-context pretrain }
      % connects pretraining documents by their semantic similarity (\S \ref{section:link} \textit{Document Linking}) using a retriever and groups these similar documents in the same contexts by traversing the document graph (\S \ref{section:traverse} \textit{Document Graph Traversal})
    }
    \label{fig:intro}
\end{figure}

% by simply altering order of the pretraining documents, 
% show the scalability of \model and significantly improves LMs' ability of understanding and reasoning over contexts by simply changing the pretraining documents ordering, which is scalable and simple.
% while the simplicity and scalability of \model
% Our results  strongly suggest \model is scalable to web-scale pretraining corpus and provide compelling evidence that 
% future pretraining method should adopt \modelname when building trainig inputs.

% We observe various benefits brought by \model: (1) \textbf{enhanced in-context learning}: the \model LM demonstrates better in-context learning capabilities, with an average performance boost of +7\% on 8 in-context learning datasets. (2) \textbf{reading comprehension}: it obtains large gains on reading comprehension tasks including single document (+xx\%) and multidocument reading comprehension (+xx\%);  (3) \textbf{factuality}: it is more faithful to prior contexts (+xx\%);  (4) \textbf{long context reasoning}: It improves LMs' ability on synthesizing information over long contexts, leading to xx\% increase in performance.  (5) \textbf{retrieval augmentation}: When paired with the retrieval augmentation, \modelname is better at aggregating information from the retrieved documents and incorporating it into predictions (+xx\%). 


% (1) \textbf{enhanced in-context learning}: the \model LM demonstrates better in-context learning capabilities, with an average performance boost of +7\% on 8 in-context learning datasets. (2) \textbf{reading comprehension}: it obtains large gains on reading comprehension tasks including single document (+xx\%) and multidocument reading comprehension (+xx\%);  (3) \textbf{factuality}: it is more faithful to prior contexts (+xx\%);  (4) \textbf{long context reasoning}: It improves LMs' ability on synthesizing information over long contexts, leading to xx\% increase in performance.  (5) \textbf{retrieval augmentation}: When paired with the retrieval augmentation, \modelname is better at aggregating information from the retrieved documents and incorporating it into predictions (+xx\%). 






==> section/method.tex <==






\section{\model}
We introduce \model: a new pretraining method that groups semantically relevant documents into a coherent input context during pretraining. 
We adopt the same model architecture and pretraining objective from LLaMA~\cite{touvron2023llama, touvron2023llama2} and \textbf{only change the data processing step}. 
% It only changes the document ordering in the data preparation step while keeping the same 
As shown in Figure~\ref{fig:main}, we first identify related documents at scale to create a document graph (\S \ref{section:link}) and then build pretraining data batches that contain related documents by traversing this graph (\S \ref{section:traverse}).  Since \model is identical to existing pretraining recipes for LMs, except for changing document ordering, it can be easily integrated into existing pretraining pipelines for large-scale LMs. 
% links each document to its nearest neighbor documents determined by the retriever and remove duplicate documents from the pretraining corpus based on the retriever's similarity scores (\S \ref{section:link}). We then propose an efficient algorithm to traverse the document graph to build the input contexts that contain semantically relevant documents (\S \ref{section:traverse}). 
% We identify three guiding principles for formulating input contexts: relevance,

% Our findings demonstrate that documents within the same input context must display a certain level of similarity to maintain \textit{relevance}, yet they should not mirror one another so closely to encourage \textit{diversity}. Surprisingly, despite highly similar documents making up xx\% of the original pretraining data, their presence within the same input contexts considerably degrade the performance of LMs, suggesting the importance of our deduplication step. 
% Furthermore, we emphasize the efficacy of our document graph traversal algorithm, which guarantees comprehensive \textit{coverage} of all documents only once.
% % that our document graph traversal algorithm that ensure coverage of all documents 
% It significantly outperforms retrieval-augmented pretraining baselines that pretrains LMs on the concatenation of input query document and its retrieved documents. Such baseline  inadvertently results in redundant training on the same documents multiple times, when a document is retrieved as a neighbor for different query documents, thereby drastically diminishing pretraining efficiency. 

% \sewon{I think this section only talks about preprocessing (how to prepare the data). Is it right? In that case, should we mention it explicitly, and that the way the model is trained and the objective and such are exactly identical to standard training? (Or we could have the training/objective as Section 3.3?)}

\sewon{I think ``creating a document graph'' is more on Sec 3.1, and Sec 3.1 is mainly about how to compute similarity search? Also, I think it might be more useful to give more overview. People might be confused why we are creating a document graph.}
\sewon{I still think describing the knn approach first (since it is a more trivial, and more intuitive method), then describe what the problems are with it, and then describe the document traverse method. Without explaining a more naive method and what their problems are, I think it's hard for readers to understand the purpose of the document graph.}
\sewon{Another random Q: have we tried a more naive baseline like iteratively choosing the top k documents from the index until we ran out of the data?}


\subsection{\textbf{Finding Related Documents At Scale}: Document Linking by Retrieval} 
\label{section:link}
To find related documents at scale, we employ a retriever model to link each document to its semantically relevant documents (\textbf{Retrieval}). We then represent the pretraining corpus as a document graph,
$\mathcal{G} =(\mathcal{D}, \mathcal{L})$ where $\mathcal{D}=\{d_i\}$ denotes a set of pretraining documents and $ \mathcal{L}$ is a set of links connecting related documents.  
% As a byproduct of the retrieval step, we compute pairwise document similarity, which later we levegrae to remove near-duplicate documents from the pretraining corpus.
As a byproduct of the retrieval step, we compute pairwise document similarity. We then leverage this similarity to remove near-duplicate documents from the pretraining corpus (\textbf{Deduplication}). \sewon{I know deduplication was really critical in person, but somehow highlighting it as a method sounds little bit odd... how about we just briefly mention (details in appendix) and hint this is very important as later ablation shows?}

% the final step, we remove duplicate documents from the pretraining corpus using the retrieval scores (\textbf{Deduplication}). 
% \nascomment{not clear why you would have duplicates in the graph if every node in the graph is a document}
% For each document $d_i \in \mathcal{D}$, we use a retriever to retrieve its k nearest neighbor documents, denoted as $N(d_i)$. 
% retrieve its k nearest neighbor documents $N(d_i)$ in $\mathcal{D}$ using a retriever. 
% We then establish links between $d_i$ and each of its k-nearest neighbors, resulting in a set of links $ \mathcal{L} = \{l_{ij} | l_{ij} = (d_i, d_j), d_i \in D, d_j \in N(d_i) \}$. 

\paragraph{Retrieval} For the retrieval process, we use a dense retriever.  Specifically,  the retriever 
maps each document $d_i \in \mathcal{D}$ to an embedding $\textbf{E}(d_i)$ by taking the mean pooling of the last hidden representation from contriever~\citep{izacard2022unsupervised} over the tokens in $d_i$. The similarity between a pair of documents is computed by their cosine similarity:
\begin{align}
s(d_i, d_j) = \cos (\textbf{E}(d_i), \textbf{E}(d_j))  \label{eq:sim}
\end{align}
For each document $d_i \in \mathcal{D}$, we use the retriever to retrieve its top-$k$ documents that have the highest similarity scores when compared with the document $d_i$, denoted as $N(d_i)$. To create a document graph, we then establish links between $d_i$ and each of its $k$-nearest neighbors, resulting in a set of links $ \mathcal{L} = \{l_{i \rightarrow j} \mid  d_i \in \mathcal{D}, d_j \in N(d_i) \}$. 
% \nascomment{tidied up notation to make it more standard} \weijia{not sure what is better way to denote this}
For efficient retrieval at scale, we precompute the embedding of each document $d \in \mathcal{D}$ and construct FAISS index~\citep{johnson2019billion} over these embeddings.

\paragraph{Deduplication} 

Corpora often have semantic duplicates: pairs of documents that are semantically related, yet not entirely identical.  As a byproduct of the retrieval step, we compute pairwise document similarity, which later we leverage to remove near-duplicate documents from the pretraining corpus.

Previous studies~\citep{yasunaga2023retrieval} show that retraining highly similar documents in the input contexts during training hurts multimodal models' performance. We have similar observations: When near duplicate documents are present in the same context, language models might merely copy from the prior document, leading to training instability.
% have designed dedicated methods to remove duplicates and show that this process can speed up learning without performance loss \citep{abbas2023semdedup}.  
Given that our retrieval approach inherently assesses  pairwise document similarity, 
 % As our retrieval process naturally compares pairwise document similarity,
 we can easily filter out near duplicate documents that have high cosine similarity with other documents. For example, as illustrated in the document graph in Figure~\ref{fig:main}, \textit{document 12} is excluded from pretraining because of its high similarity to \textit{document 3} (cosine similarity=1). We find this deduplication step is crucial for achieving performance of good language models (\S \ref{sec:ablation}).
 % \nascomment{not clear:  are you claiming that this is crucial \emph{in general} or just when applying our new method?  it's not at all clear why the retrieval + document graph construction would make duplication any more of a problem.  I think we need to be clear about whether deduplication is solving a problem our method introduces, or it's just a nice-to-have thing that we get easily as a byproduct of our method}
 
 % Following previous work, we also perform semantic deduplication using 
The retrieval stages ensures that documents placed in the input contexts exhibit \textit{relevance}, teaching LMs to reason across documents. Simultaneously, the deduplication stage encourages \textit{diversity} and prevents excessive similarity, avoiding a scenario where LMs merely learn to copy from prior contexts. \weijia{not sure if diversity is the right word to be used here}

% strike a balance between \textit{relevance}—preserving a degree of similarity—and \textit{diversity}—avoiding excessive similarity.

% makes sure that the documents placed in the input contexts display a certain level of similarity to maintain \textit{relevance}, yet they are not extremely similar to encourage \textit{diversity}.
\begin{figure}[t]
    \centering
        \vspace*{-13mm}

    \includegraphics[scale=0.22]{fig/main.png}
        \vspace*{-13mm}
    \caption{\textbf{Illustration of \model}.  \model first finds related documents at scale to create a document graph (\S \ref{section:link}) and then builds pretraining data batches by traversing the document graph (\S \ref{section:traverse})
    }
    \label{fig:main}
\end{figure}
\sewon{If we need to cut to align with the page limit, I think we can drop this section, move deduplication to the appendix, and say we use Contriever as a retrieval system (more details in the appendix).}

\subsection{\textbf{Building Pretraining Data Batches}: Document Graph Traversal } \label{section:traverse}
After finding related documents, our objective is to position these related documents within the same input context as well as maintain the original pretraining data distribution (i.e., keeping the same document frequency). We formulate this challenge as a path cover problem of the document graph and introduce an  algorithm to build the final training batches. 
% build training batches by traversing the document graph.
% % \weijia{what is the purpose of using document graph?}
% During our document linking phase, we connect semantically related documents, forming a document graph over the pretraining corpus. To facilitate language models in learn to reason over prior contexts, we aim to position semantically linked documents within the same input context as well as cover all documents from the pretraining corpus in the pretraining stage.  This can be formulated as a path cover problem of the document graph, for which we introduce an effective algorithm.
\input{iclr2023/algorithm/alg1}

\paragraph{Path cover problem}
Given the document graph $\mathcal{G} =(\mathcal{D}, \mathcal{L})$, a path cover is a set of vertex-disjoint paths such that every vertex (i.e., document $d \in \mathcal{D}$) is included in exactly one path. Note that a path cover may include paths of length 0 (i.e., an orphan document). To ensure complete coverage of all documents while placing relevant documents in training inputs, our objective is to (1) find a path cover of the document graph and (2) minimize the number of orphan documents. 

We propose a greedy algorithm to solve this problem. 
Algorithm \ref{alg1} shows the process of building a list of paths that can cover the entire document graph.
% To build one path, the algorithm starts from documents with minimum degrees and then greedily moving to unvisited neighboring documents until no such neighbors are left. This process is repeated until there are still unvisited documents. 
To construct a single path, the algorithm starts by selecting an unvisited document with minimum degrees (i.e., $Degree(d_i) = |\{ l_{ij} \in \mathcal{L} \mid d_i \in \mathcal{D} \}|
$) as the starting point for the current path because such documents are difficult to reach and more likely to become orphaned. This algorithm then incrementally expands the current path by moving to its unvisited neighboring documents, integrating the first unvisited neighbor into the current path. This process of expansion continues until all neighboring documents have been visited. Our path cover algorithm traverses the document graph, visiting each document once. Therefore, it preserves the \textit{original frequency} of documents from pretraining corpus that are later used for constructing the input contexts.


\paragraph{Merging Paths}
While our proposed algorithm reduces the number of orphan documents during the path cover construction, some orphan documents will still remain. To further reduce the number of orphan documents, we merge them into the paths of their nearest neighboring documents. 

As a final step, we concatenate documents within the same path into a long sequence, which is then truncated to create fixed-sized input contexts suitable for pretraining. The set of input texts are shuffled globally prior to being introduced to the language model training. This approach ensures \textit{relevance} within individual input contexts and fosters \textit{diversity} among input contexts within the same batches. 

% \weijia{is this paragraph necessary?}

% \nascomment{the way you're describing it, we basically are ordering all documents into one sequence.  you don't say aything about breaking that sequence into batches of the right size, or about ordering across those batches ... is there some randomization there?  seems important}

 
% A path cover of a 
%
% ensure each document is included once, guaranteeing comprehensive coverage of the entire corpus.

% Our document linking step connects semantically similar documents together, leading to a document graph over the pretraining corpus. To make language models learn to reason across relevant documents, we aim to place the linked documents together in the same input context as well as include all documents exactly once to have coverage over all documents.

% The goal is to put linked documents in the 
% After we build the document graphs, 
% We traverse 
% cover all doucments --> traverse the graph. 
% path cover problem



==> table/factual.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lcc}
\toprule
Method       & Conflict & Memotrap  \\
\midrule
\baseline       & 39.6              & 48.4     \\
kNN          & 42.1              & 54.3   \\
\modelname   & 45.8              & 56.2      \\
\bottomrule
\end{tabular}
\caption{Results on knowledge conflict datasets.} \label{tbl: factual}
\end{table}
